NoiseNCA: Noisy Seed Improves Spatio-Temporal Continuity of Neural Cellular Automata

Neural Cellular Automata (NCA) is a class of Cellular Automata where the update rule is parameterized by a neural network that can be trained using gradient descent. In this paper, we focus on NCA models used for texture synthesis, where the update rule is inspired by partial differential equations (PDEs) describing reaction-diffusion systems. To train the NCA model, the spatio-temporal domain is discretized, and Euler integration is used to numerically simulate the PDE. However, whether a trained NCA truly learns the continuous dynamic described by the corresponding PDE or merely overfits the discretization used in training remains an open question. We study NCA models at the limit where space-time discretization approaches continuity. We find that existing NCA models tend to overfit the training discretization, especially in the proximity of the initial condition, also called "seed". To address this, we propose a solution that utilizes uniform noise as the initial condition. We demonstrate the effectiveness of our approach in preserving the consistency of NCA dynamics across a wide range of spatio-temporal granularities. Our improved NCA model enables two new test-time interactions by allowing continuous control over the speed of pattern formation and the scale of the synthesized patterns. We demonstrate this new NCA feature in our interactive online demo. Our work reveals that NCA models can learn continuous dynamics and opens new venues for NCA research from a dynamical system's perspective.

==> sections/dynamical.tex <==
\section{NCA as Dynamical Systems}
We have demonstrated that our \textit{Noise-NCA} behaves better than \textit{Vanilla-NCA} and \textit{PE-NCA} at both space and time limits. Such results suggest that \textit{Noise-NCA} captures the underlying dynamics instead of overfitting to the discretization during training. We believe that this property renders \textit{Noise-NCA} a dynamical system and thus allows analysis of the model from a dynamical system perspective. Here, we conduct an experiment on measuring the maximal Lyapunov exponent (MLE) of \textit{Noise-NCA}. In the dynamical system theory, MLE is defined as the exponential rate of separation of infinitesimally close trajectories. Specifically, given an initial diverge $\delta Z_0$, MLE $\lambda$ is defined as:
\begin{equation}
    \lambda = \lim_{t \to \infty} \lim_{\delta Z_0 \to 0} \frac{1}{t} \log \left |\frac{\delta Z_t}{\delta Z_0} \right|
\end{equation}
For a discrete system described by the recurrence $x^{t+1}=f(x^t)$, MLE can be estimated by:

\begin{equation}
    \lambda = \lim_{T \to \infty} \frac{1}{T} \sum^{T}_{t=0} \log \left | f'(x^t) \right|
\end{equation}
Following Equation~\ref{eq:pde}, the MLE of \textit{Noise-NCA} can be measured by:

\begin{equation}
\begin{aligned}
    \lambda &= \lim_{T \to \infty} \frac{1}{T} \sum^{T}_{t=0} \log \left | \frac{\partial S}{\partial t} \right| \\
    &= \lim_{T \to \infty} \frac{1}{T} \sum^{T}_{t=0} \log \left | f_\theta (\State, \nabla_{\mathrm{x}}\State, \nabla_{\mathrm{y}} \State, \nabla^2 \State ) \right|
\end{aligned}
\label{eq:mle-nca}
\end{equation}

We measure MLE of \textit{Noise-NCA} on four textures, \textit{bubbly\_0101, chequered\_0121, interlaced\_0172, cracked\_0085}. We set $T=50$ and vary $\Delta t$ in range $[10^{-3}, 10^{0}]$. For each texture, $\lambda$ is measured separately for different $\Delta t$. Figure~\ref{fig:lya-esimate} shows the results.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/lya.png}
    \caption{Maximal Lyapunov exponent estimation on four textures. }
    \label{fig:lya-esimate}
\end{figure}
$\sigma_{best}$ indicates the best noise level of each \textit{Noise-NCA} model. Regardless of different noise levels and target textures, all \textit{Noise-NCA} models show internal consistency in estimating the MLE $\lambda$. The results demonstrate that MLE, a dynamical system property, can be reliably estimated from trained \textit{Noise-NCA} models, strengthening the link between \textit{Noise-NCA} and dynamical systems. Moreover, all textures have negative MLEs, implying the stability of \textit{Noise-NCA} after training. The results are in line with the empirical stability of \textit{Noise-NCA} since it generates correct textures with random seeds and under perturbations.
